Design and implementation of a modular interior-point solver for linear optimization

This paper introduces the algorithmic design and implementation of Tulip, an open-source interior-point solver for linear optimization. It implements a regularized homogeneous interior-point algorithm with multiple centrality corrections, and therefore handles unbounded and infeasible problems. The solver is written in Julia, thus allowing for a flexible and efficient implementation: Tulip's algorithmic framework is fully disentangled from linear algebra implementations and from a model's arithmetic. In particular, this allows to seamlessly integrate specialized routines for structured problems. Extensive computational results are reported. We find that Tulip is competitive with open-source interior-point solvers on the H. Mittelmann's benchmark of barrier linear programming solvers. Furthermore, we design specialized linear algebra routines for structured master problems in the context of Dantzig-Wolfe decomposition. These routines yield a tenfold speedup on large and dense instances that arise in power systems operation and two-stage stochastic programming, thereby outperforming state-of-the-art commercial interior point method solvers. Finally, we illustrate Tulip's ability to use different levels of arithmetic precision by solving problems in extended precision.

==> tex/linalg.tex <==
\section{Specialized linear algebra}
\label{sec:linalg}

In this section, we present a specialized linear algebra implementation that exploits the intrinsic structure of the master problem in a Dantzig-Wolfe decomposition.
In Section \ref{sec:linalg:DW}, we introduce the Dantzig-Wolfe decomposition principle, together with the column-generation method.
For a thorough overview of column-generation methods and their use within decomposition frameworks, we refer to \cite{Desaulniers2006column}.
A specialized Cholesky factorization is described in Section \ref{sec:linalg:cholesky}.
Computational results will be presented in Section \ref{sec:res:colgen}.



\subsection{Dantzig-Wolfe decomposition and column generation}
\label{sec:linalg:DW}

	We consider a mixed-integer linear program of the form
	\begin{align}
		\label{eq:P_objective}
		(MILP) \ \ \ \min_{x_{1}, \dots, x_{R}} \ \ \  & \sum_{r=1}^{R} c_{r}^{T} x_{r}\\
		\label{eq:P_linking}
		s.t. \ \ \ & \sum_{r=1}^{R} A_{r} x_{r} = b_{0},\\
		\label{eq:P_local}
		& x_{r} \in \mathcal{X}_{r} \ \ \ \forall r,
	\end{align}
	where $R > 0$, $c_{r}, x_{r} \in \mathbb{R}^{n_{r}}$, $b_{0} \in \mathbb{R}^{m_{0}}$, $A_{r} \in \mathbb{R}^{m_{0} \times n_{r}}$ and, for each $r$, $\mathcal{X}_{r} \subset \mathbb{R}^{n_{r}}$ is defined by a finite number of linear constraints plus integrality requirements on some coordinates of $x_{r}$.
	For ease of reading, we assume that $\mathcal{X}_{r}$ is bounded, and denote $\Omega_{r}$ the (finite) set of its extreme points.
	Therefore, we have
	\begin{align}
		conv(\mathcal{X}_{r}) = conv(\Omega_{r}) = 
		\left\{
			\sum_{\omega \in \Omega_{r}} \lambda_{\omega} \omega
			\ \middle| \ 
			e^{T} \lambda = 1,
			\lambda \geq 0
		\right\}.
	\end{align}
	
	
	The Dantzig-Wolfe decomposition principle \cite{Dantzig1960} then consists in replacing $x_{r}$ by a convex combination of extreme vertices $\{ \omega \}_{\omega \in \Omega_{r}}$.
	This change of variable yields the extended \emph{Master Problem}
	\begin{align}
		\label{eq:MP_objective}
		(MP) \ \ \ \min_{\lambda} \ \ \  & \sum_{r, \omega \in \Omega_{r}} c_{r, \omega} \lambda_{r, \omega} \\	
		\label{eq:MP_convexity}
		s.t. \ \ \ 
		& \sum_{\omega \in \Omega_{r}} \lambda_{r, \omega} =1, \ \ \ \forall r\\
		\label{eq:MP_linking}
		& \sum_{r, \omega \in \Omega_{r}} a_{r, \omega} \lambda_{r, \omega} = b_{0},\\	
		\label{eq:MP_positive}
		& \lambda \geq 0,
	\end{align}
	where $c_{r, \omega} = c_{r}^{T} \omega$ and $a_{r, \omega} = A_{r} \omega$.
	The Master Problem \eqref{eq:MP_objective}-\eqref{eq:MP_positive} contains $m_{0}+R$ constraints and $N=\sum_{r} |\Omega_{r}|$ variables, with $N$ exponentially large in general.
	Therefore, $(MP)$ is typically solved by column generation, wherein only a small subset of the variables are considered.
	Additional variables are generated iteratively by solving an auxiliary pricing problem.
	For the case at hand, we focus on the resolution of $(MP)$, i.e., we only consider the root node in a branch-and-price algorithm.
	Furthermore, we consider the case where $R$ is large compared to the number of linking constraints \eqref{eq:MP_linking}, and the vectors $a_{r, \omega}$ are dense.
	This latter assumption will be discussed in Section \ref{sec:res:colgen}.
	
	
	For each $r$, let $\bar{\Omega}_{r}$ be a (small) subset of $\Omega_{r}$.
	The \emph{Restricted Master Problem} is then defined as
	\begin{align}
		\label{eq:RMP_objective}
		(RMP) \ \ \ \min_{\lambda} \ \ \  & \sum_{r, \omega \in \bar{\Omega}_{r}} c_{r, \omega} \lambda_{r, \omega}\\	
		\label{eq:RMP_convexity}	
		s.t. \ \ \ 
		& \sum_{\omega \in \bar{\Omega}_{r}} \lambda_{r, \omega} =1, \ \ \ \forall r && [\sigma_{r}]\\
		\label{eq:RMP_linking}
		& \sum_{r, \omega \in \bar{\Omega}_{r}} a_{r, \omega} \lambda_{r, \omega}= b_{0}, && [\pi]\\	
		\label{eq:RMP_positive}
		& \lambda \geq 0.
	\end{align}
	Dual variables are indicated in brackets for each constraint.
	In all that follows, we assume that $(RMP)$ is feasible.
	If necessary, one can enforce feasibility by adding artificial variables \cite{Desaulniers2006column}.
	
	
	At the beginning of each iteration, $(RMP)$ is solved to optimality, yielding a dual solution $(\pi, \sigma)$.
	Then, for each $r$, a variable $\lambda_{r, \omega}$ with most negative reduced cost can be obtained by solving the pricing subproblem
	\begin{align}
		(SP_{r}) \ \ \ \min_{x_{r}} \ \ \  & (c_{r}^{T}  - \pi^{T}A)x_{r} - \sigma_{r}\\
		s.t. \ \ \ & x_{r} \in \mathcal{X}_{r}.
	\end{align}
	Note that $(SP_{r})$ is a mixed-integer linear program, which we assume can be solved efficiently.
	Let $z^{*}$ and $\omega^{*}$ denote the optimal value and an optimal solution of $(SP_{r})$, respectively.
	If $z^{*} < 0$, then the corresponding variable $\lambda_{r, \omega^{*}}$ has negative reduced cost and it is added to the restricted master problem.
	Otherwise, all variables $\{ \lambda_{r, \omega} \}_{\omega \in \Omega_{r}}$ have non-negative reduced cost.
	The column-generation algorithm continues until no variable with negative reduced cost can be identified among all $R$ subproblems.
	When this is the case, the current solution of $(RMP)$ is also optimal for $(MP)$, and the algorithm stops.
	A basic column-generation procedure is formally stated in Algorithm \ref{alg:colgen}.
	
	
	\begin{algorithm}[H]
		\small
		\begin{algorithmic}[1]
			\REQUIRE Initial $(RMP)$
			
			\WHILE{stopping criterion not met}
				
				\STATE Solve $(RMP)$ and obtain optimal dual variables $(\pi, \sigma)$
				
				\vspace{5pt}
				
				\STATE \COMMENT{\emph{Pricing step}}
				\FORALL{$r \in \{1, \dots, R \}$}
					\STATE Solve $SP_{r}$ with the query point $(\pi, \sigma_{r})$; obtain $\omega^{*}$
					\IF{$\bar{c}_{r,\omega^{*}} < 0$}
						\STATE Add corresponding column to $(RMP)$
					\ENDIF
				\ENDFOR
				
				\vspace{5pt}
				
				\STATE \COMMENT{\emph{Stopping criterion}}
				\IF{no column added to $(RMP)$}
					\STATE STOP
				\ENDIF
			\ENDWHILE
		\end{algorithmic}
		\caption{Column-generation procedure}
		\label{alg:colgen}
	\end{algorithm}
	

\subsection{Specialized Cholesky factorization}
\label{sec:linalg:cholesky}
    
    We now describe a specialized Cholesky factorization that exploits the block structure of the master problem.
    For ease of reading, and noting that $(MP)$ and $(RMP)$ have identical block structures, in what follows, we consider the case of $(MP)$.
	
	First, the constraint matrix of $(MP)$ is unit block-angular, i.e., it has the form
	\begin{align}
		\label{eq:struct_A_unitblockangular}
		A & = 
		\begin{bmatrix}
			e^{T} 	& \\
								& \ddots \\
								&		 & e^{T}\\
			\tilde{A}_{1} 		& \cdots & \tilde{A}_{R}
		\end{bmatrix},
	\end{align}
	where each dense lower block $\tilde{A}_{r}$ is given by
	\begin{align}
		\tilde{A}_{r} &=
		\begin{pmatrix}
			|					& 		& |\\
			a_{r, \omega_{1}}	& \dots & a_{r, \omega_{|\Omega_{r}|}}\\
			| 					&		& |
		\end{pmatrix}
		\in \mathbb{R}^{m_{0} \times |\Omega_{r}|}
		.
	\end{align}
	
	
	Let us recall that the normal equations system writes
	\[
		(A \Theta A^{T}) v = \xi,
	\]
	where $v \in \mathbb{R}^{m_{0}}$, and $\Theta \in \mathbb{R}^{N \times N}$ is a diagonal matrix with positive diagonal.
	In particular, $\Theta$ can be partitioned in blocks corresponding to the lower blocks of $A$, i.e.,
		\begin{align}
		\label{eq:struct_D_blockdiagonal}
		\Theta = 
		\begin{pmatrix}
			\Theta_{1}	& 		 & \\
						& \ddots	 & \\
						& 		 & \Theta_{R}\\
		\end{pmatrix}
		,
	\end{align}
	with $\Theta_{r} = Diag(\theta_{r})$ and $\theta_{r} > 0$.
	Consequently, the normal equations system has the form
	\begin{align}
		\label{eq:normalEq_blocks}
		\begin{bmatrix}
			e^{T} \theta_{1} 		& 			& 							& (\tilde{A}_{1}\theta_{1})^{T}\\
									& \ddots 	&							& \vdots\\
									&			& e^{T} \theta_{R} 			& (\tilde{A}_{R}\theta_{R})^{T}\\
			\tilde{A}_{1}\theta_{1} 	& \cdots 	& \tilde{A}_{R}\theta_{R} 	& \Phi
		\end{bmatrix}
		\begin{bmatrix}
			v_{1}\\
			\vdots\\
			v_{R}\\
			v_{0}
		\end{bmatrix}
		&=
		\begin{bmatrix}
			\xi_{1}\\
			\vdots\\
			\xi_{R}\\
			\xi_{0}
		\end{bmatrix},
	\end{align}
	where $v_{1}, \dots, v_{R} \in \mathbb{R}$, $v_{0} \in \mathbb{R}^{m_{0}}$, and $\Phi = \sum_{r} \tilde{A}_{r} \Theta_{r} \tilde{A}_{r}^{T} \in \mathbb{R}^{m_{0} \times m_{0}}$.
	
	
	Then, define
	\begin{align}
		l_{r} & = \frac{1}{e^{T}\theta_{r}} \tilde{A}_{r} \theta_{r} \in \mathbb{R}^{m_{0}}
	\end{align}
	and
	\begin{align}
		\label{eq:schur_complement}
		C &= \Phi - \sum_{r=1}^{R} \frac{1}{e^{T} \theta_{r}} (\tilde{A}_{r} \theta_{r}) (\tilde{A}_{r} \theta_{r})^{T} \in \mathbb{R}^{m_{0} \times m_{0}}.
	\end{align}
	Given that both $A\Theta A^{T}$ and its upper-left block are positive definite, so is the Schur complement $C$.
	Therefore, its Cholesky factorization exists, which we denote $C = L_{C} D_{C} L_{C}^{T}$.
	It then follows that a Cholesky factorization of $A \Theta A^{T}$ is given by 
	\begin{align}
		A \Theta A^{T} & = 
		\underbrace{
		\begin{bmatrix}
			1 & \\
				& \ddots \\
				&	& 1\\
			l_{1} & \cdots & l_{R} & L_{C}
		\end{bmatrix}
		}_{L}
		\times
		\underbrace{
		\begin{bmatrix}
			e^{T} \theta_{1} & & \\
				& \ddots 	&	\\
				&	& e^{T} \theta_{R} \\
			 &  & & D_{C}
		\end{bmatrix}
		}_{D}
		\times
		\underbrace{
		\begin{bmatrix}
			1 & \\
				& \ddots \\
				&	& 1\\
			l_{1} & \cdots & l_{R} & L_{C}
		\end{bmatrix}^{T}
		}_{L^{T}}
		.
	\end{align}


	Finally, once the Cholesky factors $L$ and $D$ are computed, the normal equations \eqref{eq:normalEq_blocks} are solved as follows:
	\begin{align}
		\label{eq:normalEq_globalSolve}
		v_{0} &= (L_{C} D_{C} L_{C}^{T})^{-1} \left( \xi_{0} - \sum_{r=1}^{R} \xi_{r} l_{r} \right), \\
		\label{eq:normalEq_localSolve}
		\forall r, \ v_{r} &= \dfrac{1}{e^{T}\theta_{r}} \xi_{r} - l_{r}^{T} v_{0}.
	\end{align}
	
	
	Exploiting the structure of $A$ yields several computational advantages.
	First, the factors $L$ and $D$ can be computed directly from $A$ and $\Theta$, i.e., the matrix $A \Theta A^{T}$ does not need to be explicitly formed nor stored, thus saving both time and memory.
	Second, the sparsity structure of $L$ is known beforehand.
	Specifically, the lower blocks $l_{1}, \dots, l_{R}$ are all dense column vectors, and the Schur complement $C$ is a dense $m_{0}\times m_{0}$ matrix.
	Therefore, one does not need a preprocessing phase wherein a sparsity-preserving ordering is computed, thus saving time and making memory allocation fully known in advance.
	Third, since most heavy operations are performed on dense matrices, efficient cache-exploiting kernels for dense linear algebra can be used, further speeding-up the computations.
	Finally, note that most operations such as forming the Cholesky factors and performing the backward substitutions, are amenable to parallelization.
	
	
